Geo-ConvGRU: Geographically Masked Convolutional Gated Recurrent Unit for Bird-Eye View Segmentation

Convolutional Neural Networks (CNNs) have significantly impacted various computer vision tasks, however, they inherently struggle to model long-range dependencies explicitly due to the localized nature of convolution operations. Although Transformers have addressed limitations in long-range dependencies for the spatial dimension, the temporal dimension remains underexplored. In this paper, we first highlight that 3D CNNs exhibit limitations in capturing long-range temporal dependencies. Though Transformers mitigate spatial dimension issues, they result in a considerable increase in parameter and processing speed reduction. To overcome these challenges, we introduce a simple yet effective module, Geographically Masked Convolutional Gated Recurrent Unit (Geo-ConvGRU), tailored for Bird's-Eye View segmentation. Specifically, we substitute the 3D CNN layers with ConvGRU in the temporal module to bolster the capacity of networks for handling temporal dependencies. Additionally, we integrate a geographical mask into the Convolutional Gated Recurrent Unit to suppress noise introduced by the temporal module. Comprehensive experiments conducted on the NuScenes dataset substantiate the merits of the proposed Geo-ConvGRU, revealing that our approach attains state-of-the-art performance in Bird's-Eye View segmentation.

==> Rebuttal-Round1.tex <==
\onecolumn

\noindent %We thank the editor and reviewers for their valuable comments. We have revised now the paper based on these comments.

\begin{answereditor}{ I believe the topic of your paper is interesting and beneficial to TIV, therefore I would like to invite you to revise thoroughly according to our review reports, and resubmit your revision as a New paper. If you do so, please let me know before your submission and provide me with a detailed report on your revision, I will let you know my opinion.}
We thank the Editor-in-Chief and reviewers for their suggestions. We have now revised the paper based on all the valuable comments from reviewers and have uploaded an itemized response file to help the reviewers and editors to understand where and how each comment is addressed in the revised version. 
\end{answereditor}

\begin{answerreviewer}
\qa{Supplement experimental results on the efficiency of algorithm operation and compare with other methods}{
Thanks for your suggestion. We add efficiency metrics comparison on Table~\ref{tab:ab}. Moreover, the related discussion about accuracy and efficiency has been added, "The 3D convolution from Fiery~\cite{hu2021fiery} is utilized as the baseline for this study. To ensure a fair comparison, the temporal field remains fixed at 3. According to the top section of Table~\ref{tab:ab}, ConvGRU significantly outperforms other methods, except for BEVFormer~\cite{li2022bevformer}. However, integrating a transformer structure results in considerable increases in training time and a marked decrease in FPS, which are deemed unacceptable. When considering the trade-off between accuracy and efficiency, ConvGRU emerges as a more viable selection.", in~\refcm{R1Q1}.   }

\qa{ Supplement the quantitative results of the method for long time series tasks, as this is the contribution point of the method in this paper.}{
Thanks for you suggestion.  Long-time series experiment results are reported in Table~\ref{tab:ab}. Concurrently, the influence of time series length and the reasoning behind setting the temporal field to 5 are discussed,
"Furthermore, the outcomes of long time-series tasks are presented at the bottom of Table~\ref{tab:ab}. Notably, the performance of Geo-ConvGRU improves with the addition of more previous frames. Nevertheless, long-time series result in increased training time and slower FPS, unsuitable for the real-time demands of autonomous driving. Balancing accuracy and efficiency demands, a temporal field setting of 5 is deemed optimal.", in \refcm{R1Q2}.
}

\qa{The qualitative effect video of the supplementary method in this article should be uploaded as an attachment, and there should be a comparison with other methods in the video.
}{
Appreciation is extended for the provided suggestion. A supplementary video has been added to illustrate a comparison between the proposed method and Fiery. This video is included in the current revision.
}
\end{answerreviewer}

\begin{answerreviewer}
\qa{Fig1: Please clarify what was the task. Also, clarify the meaning of the Time axis, why the unit is in hours?}{
Thanks for pointing this out.  The results depicted in Fig~\ref{fig:temporal} are based on BEV semantic segmentation. The time axis represents the model's training time on a specific temporal field, reflecting its efficiency. We change "time" to "Training time" to clarify the time axis. Moreover, the caption of Fig~\ref{fig:temporal} is updated in the revision.
}

\qa{P2 L50 "to balance the influence of pixels that are none..." You mean non-visible pixels in camera images?}{
Thanks for your professional suggestion. We modify "pixels that are none during the BEV projection process" to "non-visible pixels" in~\refcm{R2Q2}.
}

\qa{ P3 L53 "based on our thorough ablation study" also L20 "thereby confidently addressing this issue" please use more objective words.}{Thanks for your suggestion.
We change "based on our thorough ablation study" to "A comprehensive ablation study reveals a subtle inclination of the model to occasionally generate incorrect predictions concerning moving cars."(~\refcm{R2Q3-1}) and  "thereby confidently addressing this issue" to "Nonetheless, the development of a distinctive geographical mask has been successful. This mask enhances the impact of valid voxels while concurrently suppressing others, thus systematically addressing the mentioned issue."(~\refcm{R2Q3-2})
}

\qa{The Geo mask worths more clarification. 'For the geometry mask $M_{geo}$, the value of the voxel v is set to 1 if there exists a point in this voxel' Do you mean if the point in the BEV frame is visible in any camera?
}{Thanks for your professional suggestion.
To clarify this point, we modify 'For the geometry mask $M_{geo}$, the value of the voxel v is set to 1 if there exists a point in this voxel' to 'For the geometry mask $M_{geo}$, the value of the voxel v is set to 1 if the point in the BEV space is visible in any camera.'(\refcm{R2Q4})
}

\qa{Clarify the "Static" in TABLE III
}{Thanks for your suggestion. The static method assumes all obstacles static in the prediction horizon. We add the related description on Table~\ref{tab:ins seg} .}
\qa{Clarify the "baseline" in TABLE IV}{Thanks for your suggestion. The baseline is the 3D convolution from Fiery.
We clarify this in~\refcm{R1Q1}.}
\end{answerreviewer}

%\section*{Conclusion and Acknowledgement}

%\noindent We thank all editors and reviewers for these valuable suggestions and comments, and we have adopted them and revised the paper in the revised version. 

\clearpage
\twocolumn

